Robust Inference for Mediated Effects in Partially Linear Models

We consider mediated effects of an exposure, X on an outcome, Y, via a mediator, M, under no unmeasured confounding assumptions in the setting where models for the conditional expectation of the mediator and outcome are partially linear. We propose G-estimators for the direct and indirect effect and demonstrate consistent asymptotic normality for indirect effects when models for the conditional means of M, or X and Y are correctly specified, and for direct effects, when models for the conditional means of Y, or X and M are correct. This marks an improvement, in this particular setting, over previous `triple' robust methods, which do not assume partially linear mean models. Testing of the no-mediation hypothesis is inherently problematic due to the composite nature of the test (either X has no effect on M or M no effect on Y), leading to low power when both effect sizes are small. We use Generalized Methods of Moments (GMM) results to construct a new score testing framework, which includes as special cases the no-mediation and the no-direct-effect hypotheses. The proposed tests rely on an orthogonal estimation strategy for estimating nuisance parameters. Simulations show that the GMM based tests perform better in terms of power and small sample performance compared with traditional tests in the partially linear setting, with drastic improvement under model misspecification. New methods are illustrated in a mediation analysis of data from the COPERS trial, a randomized trial investigating the effect of a non-pharmacological intervention of patients suffering from chronic pain. An accompanying R package implementing these methods can be found at github.com/ohines/plmed.

==> Plots/het/nde_tab.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Thu Jan  7 09:50:05 2021
Beta & N & Spec & Bias\_G & Bias\_TTS & Var\_G & Var\_TTS & Theory\_Var\_G & Boot\_Var\_G \\ 
  \hline
(0,0,0) & 100 & XYM & 0.00294(0.00682) & 0.00103(0.00763) & 4.65(0.208) & 5.82(0.261) & 4.81(0.0323) & 5.03(0.035) \\ 
  (0,0,0) & 100 & XY & -0.00242(0.00714) & -0.00207(0.00762) & 5.1(0.228) & 5.81(0.26) & 4.73(0.0316) & 4.93(0.0339) \\ 
  (0,0,0) & 100 & XM & 0.00313(0.01) & 0.00134(0.0175) & 10(0.447) & 30.5(1.36) & 9.38(0.105) & 9.69(0.104) \\ 
  (0,0,0) & 100 & M & 0.826(0.0105) & 0.916(0.011) & 10.9(0.489) & 12.1(0.543) & 10.3(0.114) & 10.7(0.117) \\ 
  (0,0,0) & 100 & Y & -0.00453(0.00704) & -0.00631(0.00722) & 4.95(0.222) & 5.21(0.233) & 4.76(0.0296) & 4.94(0.0313) \\ 
  (0,0,0) & 500 & XYM & -0.0044(0.00308) & -0.00457(0.00326) & 4.76(0.213) & 5.32(0.238) & 4.81(0.0135) & 4.84(0.0147) \\ 
  (0,0,0) & 500 & XY & -0.000253(0.00318) & -0.000904(0.00329) & 5.04(0.226) & 5.4(0.241) & 4.84(0.014) & 4.86(0.0157) \\ 
  (0,0,0) & 500 & XM & 0.00466(0.00439) & 0.0058(0.00787) & 9.63(0.431) & 30.9(1.38) & 9.64(0.0585) & 9.68(0.0599) \\ 
  (0,0,0) & 500 & M & 0.865(0.00456) & 0.943(0.00465) & 10.4(0.465) & 10.8(0.484) & 10.6(0.0521) & 10.7(0.0543) \\ 
  (0,0,0) & 500 & Y & -0.00147(0.00305) & -0.00141(0.00306) & 4.65(0.208) & 4.69(0.21) & 4.74(0.0126) & 4.78(0.0142) \\ 
  (0,0,0) & 1000 & XYM & 0.000876(0.00218) & 6.34e-05(0.00227) & 4.74(0.212) & 5.15(0.23) & 4.83(0.00966) & 4.84(0.0119) \\ 
  (0,0,0) & 1000 & XY & -0.0063(0.00229) & -0.00691(0.00243) & 5.25(0.235) & 5.89(0.264) & 4.84(0.0101) & 4.84(0.0124) \\ 
  (0,0,0) & 1000 & XM & 0.00216(0.00314) & 0.00309(0.00574) & 9.84(0.44) & 32.9(1.47) & 9.72(0.0406) & 9.74(0.0425) \\ 
  (0,0,0) & 1000 & M & 0.866(0.00328) & 0.946(0.00335) & 10.8(0.483) & 11.2(0.502) & 10.6(0.0374) & 10.6(0.0398) \\ 
  (0,0,0) & 1000 & Y & 0.000141(0.00212) & 0.000158(0.00214) & 4.51(0.202) & 4.56(0.204) & 4.76(0.00836) & 4.75(0.0109) \\ 
  (1,1,1) & 100 & XYM & -0.0121(0.00748) & -0.0221(0.0101) & 5.6(0.25) & 10.3(0.459) & 5.47(0.0438) & 5.74(0.0464) \\ 
  (1,1,1) & 100 & XY & 0.00638(0.00729) & 0.00676(0.0078) & 5.31(0.238) & 6.09(0.272) & 5.04(0.0345) & 5.27(0.0364) \\ 
  (1,1,1) & 100 & XM & -0.00944(0.0112) & -0.0202(0.0224) & 12.6(0.563) & 50.3(2.25) & 11.1(0.122) & 11.5(0.123) \\ 
  (1,1,1) & 100 & M & 0.853(0.011) & 0.927(0.0145) & 12.2(0.546) & 21.1(0.945) & 11.9(0.134) & 12.4(0.139) \\ 
  (1,1,1) & 100 & Y & -0.00418(0.00758) & -0.00946(0.00845) & 5.75(0.257) & 7.15(0.32) & 5.48(0.0354) & 5.71(0.0375) \\ 
  (1,1,1) & 500 & XYM & 0.00199(0.00334) & 0.00342(0.00447) & 5.57(0.249) & 10(0.448) & 5.49(0.017) & 5.52(0.0191) \\ 
  (1,1,1) & 500 & XY & -0.00257(0.00313) & -0.00461(0.00332) & 4.89(0.219) & 5.52(0.247) & 5.11(0.0156) & 5.15(0.0175) \\ 
  (1,1,1) & 500 & XM & 0.000935(0.0049) & -0.0101(0.0104) & 12(0.537) & 53.7(2.4) & 11.6(0.0674) & 11.7(0.07) \\ 
  (1,1,1) & 500 & M & 0.86(0.00509) & 0.948(0.00609) & 13(0.581) & 18.5(0.829) & 12.4(0.0676) & 12.4(0.0695) \\ 
  (1,1,1) & 500 & Y & -0.00493(0.00324) & -0.00326(0.00359) & 5.26(0.236) & 6.43(0.288) & 5.52(0.0155) & 5.57(0.0177) \\ 
  (1,1,1) & 1000 & XYM & 0.00113(0.00234) & 0.000366(0.00313) & 5.5(0.246) & 9.78(0.438) & 5.5(0.0123) & 5.51(0.0145) \\ 
  (1,1,1) & 1000 & XY & 0.00185(0.00229) & 0.00243(0.00237) & 5.24(0.234) & 5.63(0.252) & 5.12(0.0105) & 5.14(0.0132) \\ 
  (1,1,1) & 1000 & XM & 0.00253(0.00343) & -0.00712(0.00702) & 11.8(0.526) & 49.3(2.21) & 11.7(0.0479) & 11.7(0.0504) \\ 
  (1,1,1) & 1000 & M & 0.866(0.00363) & 0.948(0.00449) & 13.2(0.589) & 20.1(0.9) & 12.4(0.0469) & 12.5(0.0499) \\ 
  (1,1,1) & 1000 & Y & 0.00184(0.00238) & 0.00215(0.00254) & 5.67(0.254) & 6.44(0.288) & 5.52(0.0111) & 5.53(0.0134) \\ 
   \hline


==> Plots/het/nide_tab.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Thu Jan  7 09:50:06 2021
Beta & N & Spec & Bias\_G & Bias\_TTS & Var\_G & Var\_TTS & Theory\_Var\_G & Boot\_Var\_G \\ 
  \hline
(0,0,0) & 100 & XYM & 0.000912(0.000732) & -1.4e-05(0.00124) & 0.0536(0.0024) & 0.153(0.00683) & 0.1(0.00345) & 0.157(0.157) \\ 
  (0,0,0) & 100 & XY & -0.000606(0.00061) & -0.00197(0.00163) & 0.0373(0.00167) & 0.267(0.012) & 0.0712(0.00295) & 0.112(0.112) \\ 
  (0,0,0) & 100 & XM & -0.000824(0.00132) & 0.00478(0.00226) & 0.174(0.00777) & 0.509(0.0228) & 0.296(0.0118) & 0.458(0.458) \\ 
  (0,0,0) & 100 & M & 0.000152(0.00113) & 0.00237(0.00223) & 0.128(0.00573) & 0.497(0.0223) & 0.233(0.00911) & 0.362(0.362) \\ 
  (0,0,0) & 100 & Y & -0.00144(0.00162) & -0.000188(0.00213) & 0.263(0.0118) & 0.455(0.0204) & 0.275(0.00669) & 0.323(0.323) \\ 
  (0,0,0) & 500 & XYM & 0.000163(0.000141) & 0.00027(0.000249) & 0.0099(0.000443) & 0.0309(0.00138) & 0.0184(0.000601) & 0.0283(0.0283) \\ 
  (0,0,0) & 500 & XY & 6.46e-05(0.000113) & 2.81e-05(0.000306) & 0.00634(0.000284) & 0.0468(0.0021) & 0.0138(0.00044) & 0.021(0.021) \\ 
  (0,0,0) & 500 & XM & -0.00053(0.000267) & 0.000107(0.000566) & 0.0356(0.00159) & 0.16(0.00716) & 0.0605(0.00216) & 0.0907(0.0907) \\ 
  (0,0,0) & 500 & M & -0.000258(0.000242) & -0.000363(0.000378) & 0.0292(0.00131) & 0.0715(0.0032) & 0.0499(0.00173) & 0.0739(0.0739) \\ 
  (0,0,0) & 500 & Y & -0.00064(0.000698) & -0.000749(0.000889) & 0.244(0.0109) & 0.395(0.0177) & 0.225(0.00273) & 0.234(0.234) \\ 
  (0,0,0) & 1000 & XYM & -0.000111(6.9e-05) & 6.99e-06(0.000119) & 0.00476(0.000213) & 0.0141(0.000632) & 0.00961(0.000314) & 0.0145(0.0145) \\ 
  (0,0,0) & 1000 & XY & 1.47e-05(5.98e-05) & 0.000137(0.000203) & 0.00357(0.00016) & 0.0412(0.00184) & 0.00701(0.000239) & 0.0105(0.0105) \\ 
  (0,0,0) & 1000 & XM & -9.4e-05(0.000122) & 0.000617(0.000299) & 0.0148(0.000664) & 0.0892(0.00399) & 0.0292(0.00095) & 0.0438(0.0438) \\ 
  (0,0,0) & 1000 & M & 0.000156(0.00011) & 0.00038(0.000178) & 0.0122(0.000545) & 0.0316(0.00141) & 0.0247(0.000822) & 0.0371(0.0371) \\ 
  (0,0,0) & 1000 & Y & 0.000888(0.000459) & 0.000683(0.000596) & 0.21(0.00941) & 0.355(0.0159) & 0.219(0.00185) & 0.223(0.223) \\ 
  (1,1,1) & 100 & XYM & 0.0153(0.00958) & 0.0205(0.0123) & 9.17(0.41) & 15(0.672) & 8(0.0735) & 8.31(8.31) \\ 
  (1,1,1) & 100 & XY & -0.0283(0.0111) & -0.0277(0.0182) & 12.3(0.552) & 33.3(1.49) & 11.8(0.134) & 12.1(12.1) \\ 
  (1,1,1) & 100 & XM & -0.00202(0.00961) & 0.00351(0.018) & 9.23(0.413) & 32.5(1.45) & 9.37(0.0957) & 9.5(9.5) \\ 
  (1,1,1) & 100 & M & 0.00735(0.00944) & 0.024(0.0134) & 8.91(0.399) & 18(0.807) & 8.29(0.0915) & 8.75(8.75) \\ 
  (1,1,1) & 100 & Y & 0.862(0.0116) & 0.956(0.0126) & 13.4(0.598) & 15.9(0.71) & 12.9(0.131) & 13.2(13.2) \\ 
  (1,1,1) & 500 & XYM & -0.00102(0.00406) & -0.00297(0.00496) & 8.25(0.369) & 12.3(0.55) & 7.89(0.031) & 7.94(7.94) \\ 
  (1,1,1) & 500 & XY & -0.00208(0.00504) & -0.00937(0.00828) & 12.7(0.569) & 34.3(1.53) & 12.4(0.0657) & 12.5(12.5) \\ 
  (1,1,1) & 500 & XM & 0.0018(0.00423) & 0.0197(0.00817) & 8.94(0.4) & 33.3(1.49) & 9.38(0.0442) & 9.06(9.06) \\ 
  (1,1,1) & 500 & M & -0.00262(0.00412) & -0.00967(0.00547) & 8.5(0.38) & 15(0.669) & 8.24(0.0427) & 8.36(8.36) \\ 
  (1,1,1) & 500 & Y & 0.864(0.00514) & 0.945(0.00535) & 13.2(0.591) & 14.3(0.641) & 13.2(0.0665) & 13.3(13.3) \\ 
  (1,1,1) & 1000 & XYM & -0.00159(0.00276) & -9.41e-05(0.00353) & 7.6(0.34) & 12.5(0.557) & 7.96(0.0224) & 8(8) \\ 
  (1,1,1) & 1000 & XY & -0.00388(0.00346) & -0.00618(0.00569) & 11.9(0.534) & 32.4(1.45) & 12.5(0.0482) & 12.5(12.5) \\ 
  (1,1,1) & 1000 & XM & -0.000137(0.00305) & 0.0122(0.00554) & 9.29(0.416) & 30.7(1.37) & 9.26(0.0307) & 8.87(8.87) \\ 
  (1,1,1) & 1000 & M & 0.00116(0.00291) & -0.00195(0.00393) & 8.48(0.38) & 15.4(0.69) & 8.23(0.0308) & 8.31(8.31) \\ 
  (1,1,1) & 1000 & Y & 0.867(0.00379) & 0.946(0.00391) & 14.3(0.641) & 15.3(0.683) & 13.3(0.0476) & 13.4(13.4) \\ 
   \hline


==> plmed-paper arxiv/Plots/het/nde_tab.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Thu Jan  7 09:50:05 2021
Beta & N & Spec & Bias\_G & Bias\_TTS & Var\_G & Var\_TTS & Theory\_Var\_G & Boot\_Var\_G \\ 
  \hline
(0,0,0) & 100 & XYM & 0.00294(0.00682) & 0.00103(0.00763) & 4.65(0.208) & 5.82(0.261) & 4.81(0.0323) & 5.03(0.035) \\ 
  (0,0,0) & 100 & XY & -0.00242(0.00714) & -0.00207(0.00762) & 5.1(0.228) & 5.81(0.26) & 4.73(0.0316) & 4.93(0.0339) \\ 
  (0,0,0) & 100 & XM & 0.00313(0.01) & 0.00134(0.0175) & 10(0.447) & 30.5(1.36) & 9.38(0.105) & 9.69(0.104) \\ 
  (0,0,0) & 100 & M & 0.826(0.0105) & 0.916(0.011) & 10.9(0.489) & 12.1(0.543) & 10.3(0.114) & 10.7(0.117) \\ 
  (0,0,0) & 100 & Y & -0.00453(0.00704) & -0.00631(0.00722) & 4.95(0.222) & 5.21(0.233) & 4.76(0.0296) & 4.94(0.0313) \\ 
  (0,0,0) & 500 & XYM & -0.0044(0.00308) & -0.00457(0.00326) & 4.76(0.213) & 5.32(0.238) & 4.81(0.0135) & 4.84(0.0147) \\ 
  (0,0,0) & 500 & XY & -0.000253(0.00318) & -0.000904(0.00329) & 5.04(0.226) & 5.4(0.241) & 4.84(0.014) & 4.86(0.0157) \\ 
  (0,0,0) & 500 & XM & 0.00466(0.00439) & 0.0058(0.00787) & 9.63(0.431) & 30.9(1.38) & 9.64(0.0585) & 9.68(0.0599) \\ 
  (0,0,0) & 500 & M & 0.865(0.00456) & 0.943(0.00465) & 10.4(0.465) & 10.8(0.484) & 10.6(0.0521) & 10.7(0.0543) \\ 
  (0,0,0) & 500 & Y & -0.00147(0.00305) & -0.00141(0.00306) & 4.65(0.208) & 4.69(0.21) & 4.74(0.0126) & 4.78(0.0142) \\ 
  (0,0,0) & 1000 & XYM & 0.000876(0.00218) & 6.34e-05(0.00227) & 4.74(0.212) & 5.15(0.23) & 4.83(0.00966) & 4.84(0.0119) \\ 
  (0,0,0) & 1000 & XY & -0.0063(0.00229) & -0.00691(0.00243) & 5.25(0.235) & 5.89(0.264) & 4.84(0.0101) & 4.84(0.0124) \\ 
  (0,0,0) & 1000 & XM & 0.00216(0.00314) & 0.00309(0.00574) & 9.84(0.44) & 32.9(1.47) & 9.72(0.0406) & 9.74(0.0425) \\ 
  (0,0,0) & 1000 & M & 0.866(0.00328) & 0.946(0.00335) & 10.8(0.483) & 11.2(0.502) & 10.6(0.0374) & 10.6(0.0398) \\ 
  (0,0,0) & 1000 & Y & 0.000141(0.00212) & 0.000158(0.00214) & 4.51(0.202) & 4.56(0.204) & 4.76(0.00836) & 4.75(0.0109) \\ 
  (1,1,1) & 100 & XYM & -0.0121(0.00748) & -0.0221(0.0101) & 5.6(0.25) & 10.3(0.459) & 5.47(0.0438) & 5.74(0.0464) \\ 
  (1,1,1) & 100 & XY & 0.00638(0.00729) & 0.00676(0.0078) & 5.31(0.238) & 6.09(0.272) & 5.04(0.0345) & 5.27(0.0364) \\ 
  (1,1,1) & 100 & XM & -0.00944(0.0112) & -0.0202(0.0224) & 12.6(0.563) & 50.3(2.25) & 11.1(0.122) & 11.5(0.123) \\ 
  (1,1,1) & 100 & M & 0.853(0.011) & 0.927(0.0145) & 12.2(0.546) & 21.1(0.945) & 11.9(0.134) & 12.4(0.139) \\ 
  (1,1,1) & 100 & Y & -0.00418(0.00758) & -0.00946(0.00845) & 5.75(0.257) & 7.15(0.32) & 5.48(0.0354) & 5.71(0.0375) \\ 
  (1,1,1) & 500 & XYM & 0.00199(0.00334) & 0.00342(0.00447) & 5.57(0.249) & 10(0.448) & 5.49(0.017) & 5.52(0.0191) \\ 
  (1,1,1) & 500 & XY & -0.00257(0.00313) & -0.00461(0.00332) & 4.89(0.219) & 5.52(0.247) & 5.11(0.0156) & 5.15(0.0175) \\ 
  (1,1,1) & 500 & XM & 0.000935(0.0049) & -0.0101(0.0104) & 12(0.537) & 53.7(2.4) & 11.6(0.0674) & 11.7(0.07) \\ 
  (1,1,1) & 500 & M & 0.86(0.00509) & 0.948(0.00609) & 13(0.581) & 18.5(0.829) & 12.4(0.0676) & 12.4(0.0695) \\ 
  (1,1,1) & 500 & Y & -0.00493(0.00324) & -0.00326(0.00359) & 5.26(0.236) & 6.43(0.288) & 5.52(0.0155) & 5.57(0.0177) \\ 
  (1,1,1) & 1000 & XYM & 0.00113(0.00234) & 0.000366(0.00313) & 5.5(0.246) & 9.78(0.438) & 5.5(0.0123) & 5.51(0.0145) \\ 
  (1,1,1) & 1000 & XY & 0.00185(0.00229) & 0.00243(0.00237) & 5.24(0.234) & 5.63(0.252) & 5.12(0.0105) & 5.14(0.0132) \\ 
  (1,1,1) & 1000 & XM & 0.00253(0.00343) & -0.00712(0.00702) & 11.8(0.526) & 49.3(2.21) & 11.7(0.0479) & 11.7(0.0504) \\ 
  (1,1,1) & 1000 & M & 0.866(0.00363) & 0.948(0.00449) & 13.2(0.589) & 20.1(0.9) & 12.4(0.0469) & 12.5(0.0499) \\ 
  (1,1,1) & 1000 & Y & 0.00184(0.00238) & 0.00215(0.00254) & 5.67(0.254) & 6.44(0.288) & 5.52(0.0111) & 5.53(0.0134) \\ 
   \hline


==> plmed-paper arxiv/Plots/het/nide_tab.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Thu Jan  7 09:50:06 2021
Beta & N & Spec & Bias\_G & Bias\_TTS & Var\_G & Var\_TTS & Theory\_Var\_G & Boot\_Var\_G \\ 
  \hline
(0,0,0) & 100 & XYM & 0.000912(0.000732) & -1.4e-05(0.00124) & 0.0536(0.0024) & 0.153(0.00683) & 0.1(0.00345) & 0.157(0.157) \\ 
  (0,0,0) & 100 & XY & -0.000606(0.00061) & -0.00197(0.00163) & 0.0373(0.00167) & 0.267(0.012) & 0.0712(0.00295) & 0.112(0.112) \\ 
  (0,0,0) & 100 & XM & -0.000824(0.00132) & 0.00478(0.00226) & 0.174(0.00777) & 0.509(0.0228) & 0.296(0.0118) & 0.458(0.458) \\ 
  (0,0,0) & 100 & M & 0.000152(0.00113) & 0.00237(0.00223) & 0.128(0.00573) & 0.497(0.0223) & 0.233(0.00911) & 0.362(0.362) \\ 
  (0,0,0) & 100 & Y & -0.00144(0.00162) & -0.000188(0.00213) & 0.263(0.0118) & 0.455(0.0204) & 0.275(0.00669) & 0.323(0.323) \\ 
  (0,0,0) & 500 & XYM & 0.000163(0.000141) & 0.00027(0.000249) & 0.0099(0.000443) & 0.0309(0.00138) & 0.0184(0.000601) & 0.0283(0.0283) \\ 
  (0,0,0) & 500 & XY & 6.46e-05(0.000113) & 2.81e-05(0.000306) & 0.00634(0.000284) & 0.0468(0.0021) & 0.0138(0.00044) & 0.021(0.021) \\ 
  (0,0,0) & 500 & XM & -0.00053(0.000267) & 0.000107(0.000566) & 0.0356(0.00159) & 0.16(0.00716) & 0.0605(0.00216) & 0.0907(0.0907) \\ 
  (0,0,0) & 500 & M & -0.000258(0.000242) & -0.000363(0.000378) & 0.0292(0.00131) & 0.0715(0.0032) & 0.0499(0.00173) & 0.0739(0.0739) \\ 
  (0,0,0) & 500 & Y & -0.00064(0.000698) & -0.000749(0.000889) & 0.244(0.0109) & 0.395(0.0177) & 0.225(0.00273) & 0.234(0.234) \\ 
  (0,0,0) & 1000 & XYM & -0.000111(6.9e-05) & 6.99e-06(0.000119) & 0.00476(0.000213) & 0.0141(0.000632) & 0.00961(0.000314) & 0.0145(0.0145) \\ 
  (0,0,0) & 1000 & XY & 1.47e-05(5.98e-05) & 0.000137(0.000203) & 0.00357(0.00016) & 0.0412(0.00184) & 0.00701(0.000239) & 0.0105(0.0105) \\ 
  (0,0,0) & 1000 & XM & -9.4e-05(0.000122) & 0.000617(0.000299) & 0.0148(0.000664) & 0.0892(0.00399) & 0.0292(0.00095) & 0.0438(0.0438) \\ 
  (0,0,0) & 1000 & M & 0.000156(0.00011) & 0.00038(0.000178) & 0.0122(0.000545) & 0.0316(0.00141) & 0.0247(0.000822) & 0.0371(0.0371) \\ 
  (0,0,0) & 1000 & Y & 0.000888(0.000459) & 0.000683(0.000596) & 0.21(0.00941) & 0.355(0.0159) & 0.219(0.00185) & 0.223(0.223) \\ 
  (1,1,1) & 100 & XYM & 0.0153(0.00958) & 0.0205(0.0123) & 9.17(0.41) & 15(0.672) & 8(0.0735) & 8.31(8.31) \\ 
  (1,1,1) & 100 & XY & -0.0283(0.0111) & -0.0277(0.0182) & 12.3(0.552) & 33.3(1.49) & 11.8(0.134) & 12.1(12.1) \\ 
  (1,1,1) & 100 & XM & -0.00202(0.00961) & 0.00351(0.018) & 9.23(0.413) & 32.5(1.45) & 9.37(0.0957) & 9.5(9.5) \\ 
  (1,1,1) & 100 & M & 0.00735(0.00944) & 0.024(0.0134) & 8.91(0.399) & 18(0.807) & 8.29(0.0915) & 8.75(8.75) \\ 
  (1,1,1) & 100 & Y & 0.862(0.0116) & 0.956(0.0126) & 13.4(0.598) & 15.9(0.71) & 12.9(0.131) & 13.2(13.2) \\ 
  (1,1,1) & 500 & XYM & -0.00102(0.00406) & -0.00297(0.00496) & 8.25(0.369) & 12.3(0.55) & 7.89(0.031) & 7.94(7.94) \\ 
  (1,1,1) & 500 & XY & -0.00208(0.00504) & -0.00937(0.00828) & 12.7(0.569) & 34.3(1.53) & 12.4(0.0657) & 12.5(12.5) \\ 
  (1,1,1) & 500 & XM & 0.0018(0.00423) & 0.0197(0.00817) & 8.94(0.4) & 33.3(1.49) & 9.38(0.0442) & 9.06(9.06) \\ 
  (1,1,1) & 500 & M & -0.00262(0.00412) & -0.00967(0.00547) & 8.5(0.38) & 15(0.669) & 8.24(0.0427) & 8.36(8.36) \\ 
  (1,1,1) & 500 & Y & 0.864(0.00514) & 0.945(0.00535) & 13.2(0.591) & 14.3(0.641) & 13.2(0.0665) & 13.3(13.3) \\ 
  (1,1,1) & 1000 & XYM & -0.00159(0.00276) & -9.41e-05(0.00353) & 7.6(0.34) & 12.5(0.557) & 7.96(0.0224) & 8(8) \\ 
  (1,1,1) & 1000 & XY & -0.00388(0.00346) & -0.00618(0.00569) & 11.9(0.534) & 32.4(1.45) & 12.5(0.0482) & 12.5(12.5) \\ 
  (1,1,1) & 1000 & XM & -0.000137(0.00305) & 0.0122(0.00554) & 9.29(0.416) & 30.7(1.37) & 9.26(0.0307) & 8.87(8.87) \\ 
  (1,1,1) & 1000 & M & 0.00116(0.00291) & -0.00195(0.00393) & 8.48(0.38) & 15.4(0.69) & 8.23(0.0308) & 8.31(8.31) \\ 
  (1,1,1) & 1000 & Y & 0.867(0.00379) & 0.946(0.00391) & 14.3(0.641) & 15.3(0.683) & 13.3(0.0476) & 13.4(13.4) \\ 
   \hline


==> plmed-paper arxiv/Plots/hom/nde_tab.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Thu Jan  7 09:50:03 2021
Beta & N & Spec & Bias\_G & Bias\_TTS & Var\_G & Var\_TTS & Theory\_Var\_G & Boot\_Var\_G \\ 
  \hline
(0,0,0) & 100 & XYM & 0.00205(0.00718) & -0.00188(0.0077) & 5.15(0.23) & 5.92(0.265) & 4.76(0.0327) & 4.97(0.035) \\ 
  (0,0,0) & 100 & XY & -0.000128(0.00708) & -0.00336(0.00737) & 5.01(0.224) & 5.44(0.243) & 4.75(0.0327) & 4.94(0.0347) \\ 
  (0,0,0) & 100 & XM & 0.0171(0.00974) & 0.0147(0.016) & 9.49(0.425) & 25.6(1.15) & 9.37(0.115) & 9.64(0.111) \\ 
  (0,0,0) & 100 & M & 0.843(0.0104) & 0.932(0.0112) & 10.9(0.488) & 12.5(0.558) & 10.2(0.108) & 10.6(0.111) \\ 
  (0,0,0) & 100 & Y & -0.00524(0.00728) & -0.0053(0.00738) & 5.3(0.237) & 5.45(0.244) & 4.72(0.0299) & 4.89(0.0319) \\ 
  (0,0,0) & 500 & XYM & 0.00409(0.00311) & 0.00318(0.00327) & 4.83(0.216) & 5.35(0.239) & 4.84(0.0142) & 4.88(0.0156) \\ 
  (0,0,0) & 500 & XY & 0.00205(0.00308) & 0.00241(0.0032) & 4.73(0.212) & 5.12(0.229) & 4.82(0.0133) & 4.84(0.0149) \\ 
  (0,0,0) & 500 & XM & 0.00245(0.00443) & 0.00352(0.00791) & 9.8(0.438) & 31.3(1.4) & 9.69(0.0554) & 9.73(0.057) \\ 
  (0,0,0) & 500 & M & 0.861(0.00444) & 0.941(0.00456) & 9.88(0.442) & 10.4(0.464) & 10.4(0.0487) & 10.5(0.0499) \\ 
  (0,0,0) & 500 & Y & 0.0026(0.00316) & 0.00141(0.00321) & 4.99(0.223) & 5.14(0.23) & 4.79(0.0125) & 4.82(0.0143) \\ 
  (0,0,0) & 1000 & XYM & -0.00136(0.00221) & -0.00103(0.00227) & 4.87(0.218) & 5.16(0.231) & 4.85(0.00996) & 4.86(0.0123) \\ 
  (0,0,0) & 1000 & XY & 0.000526(0.00218) & 0.000912(0.00226) & 4.76(0.213) & 5.09(0.228) & 4.83(0.00941) & 4.83(0.0113) \\ 
  (0,0,0) & 1000 & XM & -0.000147(0.00309) & 0.00113(0.0051) & 9.57(0.428) & 26.1(1.17) & 9.58(0.038) & 9.59(0.0395) \\ 
  (0,0,0) & 1000 & M & 0.869(0.00331) & 0.95(0.0034) & 11(0.491) & 11.6(0.518) & 10.6(0.0383) & 10.7(0.0406) \\ 
  (0,0,0) & 1000 & Y & 0.00184(0.00216) & 0.00153(0.00221) & 4.66(0.208) & 4.88(0.218) & 4.8(0.00878) & 4.82(0.0113) \\ 
  (1,1,1) & 100 & XYM & 0.0107(0.00776) & 0.00396(0.0103) & 6.03(0.27) & 10.5(0.471) & 5.82(0.0437) & 6.11(0.0459) \\ 
  (1,1,1) & 100 & XY & -0.00412(0.00745) & -0.00188(0.00778) & 5.55(0.249) & 6.05(0.271) & 5.13(0.036) & 5.39(0.0388) \\ 
  (1,1,1) & 100 & XM & -0.0089(0.0112) & -0.0113(0.0193) & 12.4(0.557) & 37.4(1.67) & 12.2(0.152) & 12.7(0.152) \\ 
  (1,1,1) & 100 & M & 0.838(0.0115) & 0.914(0.0159) & 13.3(0.596) & 25.2(1.13) & 12.8(0.145) & 13.4(0.149) \\ 
  (1,1,1) & 100 & Y & -0.0135(0.0073) & -0.00428(0.00813) & 5.33(0.238) & 6.61(0.296) & 5.7(0.0387) & 5.95(0.0407) \\ 
  (1,1,1) & 500 & XYM & 0.00438(0.00351) & 0.00847(0.00445) & 6.14(0.275) & 9.92(0.444) & 5.85(0.0192) & 5.9(0.0211) \\ 
  (1,1,1) & 500 & XY & 0.00309(0.00316) & 0.00385(0.0033) & 4.99(0.223) & 5.44(0.243) & 5.16(0.0151) & 5.21(0.0173) \\ 
  (1,1,1) & 500 & XM & -0.00834(0.00511) & -0.00323(0.0115) & 13(0.583) & 66.5(2.98) & 12.6(0.0688) & 12.7(0.0705) \\ 
  (1,1,1) & 500 & M & 0.872(0.00511) & 0.954(0.00691) & 13(0.584) & 23.9(1.07) & 13.3(0.0709) & 13.4(0.0732) \\ 
  (1,1,1) & 500 & Y & 0.00428(0.00336) & 0.0034(0.00358) & 5.64(0.252) & 6.42(0.287) & 5.7(0.0161) & 5.75(0.0182) \\ 
  (1,1,1) & 1000 & XYM & 4.3e-05(0.00237) & -0.000762(0.00309) & 5.6(0.251) & 9.53(0.426) & 5.81(0.0138) & 5.85(0.0163) \\ 
  (1,1,1) & 1000 & XY & -8.16e-05(0.00223) & 0.000244(0.00232) & 4.98(0.223) & 5.37(0.24) & 5.16(0.0109) & 5.2(0.0131) \\ 
  (1,1,1) & 1000 & XM & 0.00194(0.00361) & 0.0103(0.00841) & 13(0.583) & 70.7(3.16) & 12.7(0.0531) & 12.7(0.0564) \\ 
  (1,1,1) & 1000 & M & 0.863(0.0037) & 0.943(0.00521) & 13.7(0.611) & 27.2(1.22) & 13.5(0.0581) & 13.6(0.061) \\ 
  (1,1,1) & 1000 & Y & 0.00272(0.00243) & 0.0014(0.00259) & 5.92(0.265) & 6.7(0.3) & 5.74(0.0115) & 5.76(0.014) \\ 
   \hline


==> plmed-paper arxiv/Plots/hom/nide_tab.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Thu Jan  7 09:50:04 2021
Beta & N & Spec & Bias\_G & Bias\_TTS & Var\_G & Var\_TTS & Theory\_Var\_G & Boot\_Var\_G \\ 
  \hline
(0,0,0) & 100 & XYM & -0.000762(0.00069) & -0.000561(0.00123) & 0.0476(0.00213) & 0.151(0.00675) & 0.0974(0.00342) & 0.154(0.154) \\ 
  (0,0,0) & 100 & XY & 0.00211(0.000644) & 0.00228(0.00151) & 0.0414(0.00185) & 0.229(0.0103) & 0.0731(0.00303) & 0.112(0.112) \\ 
  (0,0,0) & 100 & XM & 0.00241(0.00128) & 0.0055(0.0022) & 0.163(0.0073) & 0.486(0.0217) & 0.29(0.0112) & 0.445(0.445) \\ 
  (0,0,0) & 100 & M & 0.000992(0.00121) & 0.00284(0.00223) & 0.146(0.00651) & 0.497(0.0223) & 0.271(0.0101) & 0.413(0.413) \\ 
  (0,0,0) & 100 & Y & 0.00209(0.00181) & 0.00264(0.00228) & 0.328(0.0147) & 0.518(0.0232) & 0.311(0.0075) & 0.36(0.36) \\ 
  (0,0,0) & 500 & XYM & -2.61e-05(0.000136) & -0.000147(0.000248) & 0.0093(0.000416) & 0.0308(0.00138) & 0.019(0.000606) & 0.029(0.029) \\ 
  (0,0,0) & 500 & XY & 9.12e-06(0.000105) & -6.06e-06(0.000298) & 0.00556(0.000249) & 0.0445(0.00199) & 0.0125(0.000427) & 0.0192(0.0192) \\ 
  (0,0,0) & 500 & XM & -0.000496(0.000261) & -0.000989(0.000548) & 0.0341(0.00153) & 0.15(0.00673) & 0.0621(0.00217) & 0.0921(0.0921) \\ 
  (0,0,0) & 500 & M & 0.000276(0.000243) & 0.000609(0.000412) & 0.0295(0.00132) & 0.0847(0.00379) & 0.0536(0.00184) & 0.0796(0.0796) \\ 
  (0,0,0) & 500 & Y & -0.00153(0.000734) & -0.00077(0.000933) & 0.27(0.0121) & 0.436(0.0195) & 0.27(0.00291) & 0.279(0.279) \\ 
  (0,0,0) & 1000 & XYM & 2.98e-05(6.83e-05) & -0.000152(0.000112) & 0.00466(0.000209) & 0.0125(0.000561) & 0.00954(0.000296) & 0.0145(0.0145) \\ 
  (0,0,0) & 1000 & XY & -3.7e-05(5.58e-05) & -1.95e-05(0.000161) & 0.00312(0.00014) & 0.0259(0.00116) & 0.00646(0.000211) & 0.00974(0.00974) \\ 
  (0,0,0) & 1000 & XM & -2.77e-05(0.000126) & 5.37e-05(0.000268) & 0.0158(0.000706) & 0.0716(0.0032) & 0.0292(0.000954) & 0.0437(0.0437) \\ 
  (0,0,0) & 1000 & M & 4.46e-05(0.000115) & 4.94e-05(0.000194) & 0.0133(0.000594) & 0.0375(0.00168) & 0.0267(0.000878) & 0.0399(0.0399) \\ 
  (0,0,0) & 1000 & Y & -0.00055(0.000508) & -0.000439(0.000653) & 0.258(0.0115) & 0.426(0.0191) & 0.266(0.00217) & 0.269(0.269) \\ 
  (1,1,1) & 100 & XYM & 0.003(0.00743) & 0.011(0.0103) & 5.52(0.247) & 10.7(0.478) & 5.88(0.0507) & 6.16(6.16) \\ 
  (1,1,1) & 100 & XY & -0.000413(0.0103) & -0.00162(0.0178) & 10.5(0.472) & 31.7(1.42) & 9.58(0.109) & 9.8(9.8) \\ 
  (1,1,1) & 100 & XM & 0.00459(0.0093) & 0.0116(0.0145) & 8.65(0.387) & 21(0.942) & 8.03(0.0955) & 8.51(8.51) \\ 
  (1,1,1) & 100 & M & -0.00994(0.00879) & 0.0058(0.0134) & 7.73(0.346) & 17.9(0.802) & 7.39(0.0889) & 7.91(7.91) \\ 
  (1,1,1) & 100 & Y & 0.831(0.0111) & 0.921(0.0124) & 12.4(0.553) & 15.5(0.693) & 11.3(0.111) & 11.7(11.7) \\ 
  (1,1,1) & 500 & XYM & 0.000102(0.00352) & -0.00223(0.0044) & 6.19(0.277) & 9.67(0.433) & 5.84(0.0236) & 5.9(5.9) \\ 
  (1,1,1) & 500 & XY & -0.00721(0.00441) & -0.0119(0.00778) & 9.73(0.435) & 30.3(1.35) & 9.88(0.0587) & 9.9(9.9) \\ 
  (1,1,1) & 500 & XM & 0.00657(0.00394) & 0.00122(0.00917) & 7.77(0.348) & 42.1(1.88) & 7.92(0.0416) & 8.03(8.03) \\ 
  (1,1,1) & 500 & M & -0.00231(0.00376) & -0.00462(0.00599) & 7.06(0.316) & 17.9(0.803) & 7.42(0.0403) & 7.58(7.58) \\ 
  (1,1,1) & 500 & Y & 0.855(0.00516) & 0.937(0.0055) & 13.3(0.596) & 15.1(0.677) & 11.8(0.0618) & 11.8(11.8) \\ 
  (1,1,1) & 1000 & XYM & -0.00296(0.00241) & -0.00196(0.00314) & 5.83(0.261) & 9.83(0.44) & 5.84(0.0181) & 5.87(5.87) \\ 
  (1,1,1) & 1000 & XY & 0.00151(0.00319) & -0.00187(0.00545) & 10.2(0.454) & 29.7(1.33) & 9.99(0.0444) & 10(10) \\ 
  (1,1,1) & 1000 & XM & 0.00169(0.00286) & -0.00207(0.00693) & 8.18(0.366) & 48.1(2.15) & 7.89(0.0308) & 7.93(7.93) \\ 
  (1,1,1) & 1000 & M & -0.000208(0.0028) & 0.00131(0.00458) & 7.81(0.35) & 21(0.938) & 7.45(0.0309) & 7.6(7.6) \\ 
  (1,1,1) & 1000 & Y & 0.865(0.00339) & 0.946(0.00361) & 11.5(0.514) & 13.1(0.584) & 11.8(0.0447) & 11.8(11.8) \\ 
   \hline


==> plmed-paper arxiv/Plots/log/nde_tab.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Thu Jan  7 09:50:09 2021
Beta & N & Spec & Bias\_G & Bias\_TTS & Var\_G & Var\_TTS & Theory\_Var\_G & Boot\_Var\_G \\ 
  \hline
(0,0,0) & 100 & XYM & -0.00301(0.00656) & 0.00107(0.00705) & 4.31(0.193) & 4.97(0.222) & 4.77(0.0313) & 6.54(0.248) \\ 
  (0,0,0) & 100 & XY & 0.00514(0.00733) & 0.00348(0.00803) & 5.37(0.24) & 6.45(0.288) & 4.79(0.0321) & 7.62(0.303) \\ 
  (0,0,0) & 100 & XM & 0.00579(0.0101) & 0.0267(0.0184) & 10.2(0.455) & 34(1.52) & 9.3(0.122) & 12.3(0.503) \\ 
  (0,0,0) & 100 & M & 0.836(0.0105) & 0.92(0.0111) & 11(0.494) & 12.3(0.552) & 9.96(0.0995) & 80.9(1.9) \\ 
  (0,0,0) & 100 & Y & 0.00444(0.00685) & 0.00214(0.00691) & 4.69(0.21) & 4.78(0.214) & 4.59(0.0306) & 7.85(0.311) \\ 
  (0,0,0) & 500 & XYM & 0.000106(0.00301) & 0.00157(0.00314) & 4.52(0.202) & 4.94(0.221) & 4.83(0.0136) & 6.86(0.264) \\ 
  (0,0,0) & 500 & XY & 0.000599(0.00315) & 0.0014(0.00335) & 4.98(0.223) & 5.62(0.252) & 4.83(0.0139) & 6.85(0.267) \\ 
  (0,0,0) & 500 & XM & -0.00674(0.00455) & -0.00605(0.00887) & 10.4(0.464) & 39.3(1.76) & 9.64(0.0593) & 12.3(0.488) \\ 
  (0,0,0) & 500 & M & 0.862(0.00472) & 0.944(0.0048) & 11.1(0.499) & 11.5(0.515) & 10.5(0.0534) & 378(4.19) \\ 
  (0,0,0) & 500 & Y & 0.000134(0.00313) & 0.000521(0.00314) & 4.9(0.219) & 4.93(0.221) & 4.61(0.0121) & 14.2(0.497) \\ 
  (0,0,0) & 1000 & XYM & -0.00227(0.00225) & -0.00227(0.00238) & 5.07(0.227) & 5.67(0.254) & 4.83(0.00983) & 7.16(0.288) \\ 
  (0,0,0) & 1000 & XY & -0.00111(0.00221) & -0.000989(0.0023) & 4.88(0.218) & 5.28(0.236) & 4.84(0.0101) & 7.07(0.258) \\ 
  (0,0,0) & 1000 & XM & -0.00127(0.00302) & 0.000813(0.00527) & 9.12(0.408) & 27.8(1.24) & 9.64(0.0377) & 11.7(0.472) \\ 
  (0,0,0) & 1000 & M & 0.863(0.00337) & 0.942(0.0034) & 11.4(0.509) & 11.6(0.518) & 10.6(0.0371) & 742(5.98) \\ 
  (0,0,0) & 1000 & Y & -0.000594(0.00219) & -0.00018(0.00222) & 4.8(0.215) & 4.91(0.22) & 4.64(0.00849) & 21.4(0.633) \\ 
  (1,1,1) & 100 & XYM & 0.00449(0.00736) & 0.00319(0.00818) & 5.42(0.242) & 6.69(0.299) & 5.11(0.0375) & 70.7(1.34) \\ 
  (1,1,1) & 100 & XY & -0.00356(0.00714) & 0.00596(0.00833) & 5.1(0.228) & 6.95(0.311) & 4.97(0.0351) & 73.6(1.33) \\ 
  (1,1,1) & 100 & XM & 0.0209(0.0103) & -0.00588(0.0212) & 10.6(0.474) & 45.1(2.02) & 9.77(0.121) & 79.3(1.83) \\ 
  (1,1,1) & 100 & M & 0.888(0.0109) & 0.924(0.0115) & 11.9(0.534) & 13.3(0.595) & 10.9(0.108) & 298(3.81) \\ 
  (1,1,1) & 100 & Y & -0.00842(0.00693) & -0.00814(0.00754) & 4.81(0.215) & 5.69(0.255) & 5.03(0.0372) & 57.5(1.1) \\ 
  (1,1,1) & 500 & XYM & -0.000439(0.00312) & -0.000264(0.00336) & 4.87(0.218) & 5.64(0.252) & 5.06(0.0155) & 323(2.79) \\ 
  (1,1,1) & 500 & XY & -0.00397(0.0032) & -0.00326(0.00347) & 5.11(0.229) & 6.03(0.27) & 5.04(0.0154) & 336(2.86) \\ 
  (1,1,1) & 500 & XM & 0.0303(0.00452) & -0.00829(0.0084) & 10.2(0.457) & 35.3(1.58) & 10.2(0.0614) & 352(3.92) \\ 
  (1,1,1) & 500 & M & 0.901(0.00479) & 0.935(0.00495) & 11.5(0.513) & 12.3(0.548) & 11.2(0.0545) & 1460(8.46) \\ 
  (1,1,1) & 500 & Y & 0.00265(0.00313) & 0.00292(0.00328) & 4.91(0.219) & 5.38(0.241) & 5.02(0.0151) & 267(2.49) \\ 
  (1,1,1) & 1000 & XYM & -0.00664(0.0022) & -0.00507(0.00238) & 4.83(0.216) & 5.65(0.253) & 5.07(0.0111) & 629(3.77) \\ 
  (1,1,1) & 1000 & XY & -0.00122(0.00242) & -0.000419(0.00257) & 5.86(0.262) & 6.6(0.296) & 5.04(0.0108) & 675(4.3) \\ 
  (1,1,1) & 1000 & XM & 0.029(0.00318) & -0.0139(0.00569) & 10.1(0.453) & 32.4(1.45) & 10.4(0.0411) & 691(5.43) \\ 
  (1,1,1) & 1000 & M & 0.918(0.00339) & 0.951(0.00349) & 11.5(0.515) & 12.2(0.546) & 11.5(0.0405) & 2970(12.1) \\ 
  (1,1,1) & 1000 & Y & 0.000258(0.00229) & -0.000654(0.00239) & 5.24(0.234) & 5.73(0.257) & 5.05(0.0111) & 523(3.62) \\ 
   \hline


==> plmed-paper arxiv/Plots/log/nide_tab.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Thu Jan  7 09:50:10 2021
Beta & N & Spec & Bias\_G & Bias\_TTS & Var\_G & Var\_TTS & Theory\_Var\_G & Boot\_Var\_G \\ 
  \hline
(0,0,0) & 100 & XYM & -0.000386(0.000758) & 1.94e-05(0.0011) & 0.0574(0.00257) & 0.12(0.00537) & 0.0994(0.273) & 9.98(9.98) \\ 
  (0,0,0) & 100 & XY & 0.000943(0.000678) & 0.00172(0.00138) & 0.0459(0.00206) & 0.19(0.00849) & 0.0945(0.21) & 9.26(9.26) \\ 
  (0,0,0) & 100 & XM & 0.00118(0.00118) & 0.00274(0.00183) & 0.14(0.00625) & 0.336(0.015) & 0.241(0.596) & 22.5(22.5) \\ 
  (0,0,0) & 100 & M & -0.00348(0.00116) & -0.00133(0.00158) & 0.135(0.00602) & 0.251(0.0112) & 0.224(0.58) & 21.9(21.9) \\ 
  (0,0,0) & 100 & Y & -0.00104(0.00105) & -0.000516(0.00147) & 0.111(0.00495) & 0.216(0.00967) & 0.159(0.179) & 8.59(8.59) \\ 
  (0,0,0) & 500 & XYM & 0.000136(0.000144) & -0.000222(0.000225) & 0.0103(0.000461) & 0.0252(0.00113) & 0.0198(0.223) & 9.59(9.59) \\ 
  (0,0,0) & 500 & XY & -0.000105(0.000137) & -7.15e-05(0.00026) & 0.00934(0.000418) & 0.0339(0.00152) & 0.0192(0.221) & 9.3(9.3) \\ 
  (0,0,0) & 500 & XM & 0.000125(0.000217) & 0.00019(0.00033) & 0.0234(0.00105) & 0.0543(0.00243) & 0.0461(0.506) & 21.8(21.8) \\ 
  (0,0,0) & 500 & M & -0.000259(0.000191) & 0.000187(0.000271) & 0.0183(0.000817) & 0.0369(0.00165) & 0.0392(0.467) & 20.2(20.2) \\ 
  (0,0,0) & 500 & Y & 0.000414(0.000398) & 0.000288(0.000525) & 0.079(0.00354) & 0.138(0.00616) & 0.0888(0.16) & 8.2(8.2) \\ 
  (0,0,0) & 1000 & XYM & -6.41e-05(7.27e-05) & 5.69e-05(0.000113) & 0.00529(0.000237) & 0.0128(0.000571) & 0.0101(0.202) & 9.45(9.45) \\ 
  (0,0,0) & 1000 & XY & 3.72e-05(6.75e-05) & 2.97e-05(0.000135) & 0.00456(0.000204) & 0.0182(0.000813) & 0.0099(0.193) & 9.01(9.01) \\ 
  (0,0,0) & 1000 & XM & -1.45e-05(0.000103) & -9.14e-05(0.000177) & 0.0107(0.000477) & 0.0315(0.00141) & 0.0227(0.419) & 20.6(20.6) \\ 
  (0,0,0) & 1000 & M & -0.000306(0.000115) & 9.28e-05(0.000152) & 0.0133(0.000595) & 0.0231(0.00103) & 0.0224(0.506) & 21.3(21.3) \\ 
  (0,0,0) & 1000 & Y & 6.49e-05(0.00027) & -0.00032(0.000358) & 0.0727(0.00325) & 0.128(0.00572) & 0.0769(0.162) & 8.28(8.28) \\ 
  (1,1,1) & 100 & XYM & 0.0155(0.00379) & 0.00598(0.0045) & 1.44(0.0643) & 2.02(0.0905) & 1.39(1.13) & 73.4(73.4) \\ 
  (1,1,1) & 100 & XY & 0.0132(0.00346) & -0.00869(0.00528) & 1.2(0.0535) & 2.78(0.125) & 1.23(1.21) & 78.1(78.1) \\ 
  (1,1,1) & 100 & XM & -0.033(0.00366) & -0.00466(0.00569) & 1.34(0.0599) & 3.24(0.145) & 1.43(1.29) & 62.1(62.1) \\ 
  (1,1,1) & 100 & M & -0.0495(0.0036) & -0.00195(0.00502) & 1.29(0.0579) & 2.52(0.113) & 1.35(1.19) & 56.9(56.9) \\ 
  (1,1,1) & 100 & Y & 0.112(0.00395) & 0.11(0.00469) & 1.56(0.0699) & 2.2(0.0985) & 1.57(1) & 63.5(63.5) \\ 
  (1,1,1) & 500 & XYM & 0.00586(0.00163) & -0.00301(0.00181) & 1.32(0.0591) & 1.65(0.0736) & 1.26(2.43) & 322(322) \\ 
  (1,1,1) & 500 & XY & 0.0154(0.00148) & 0.00137(0.00175) & 1.1(0.0492) & 1.53(0.0683) & 1.14(2.49) & 343(343) \\ 
  (1,1,1) & 500 & XM & -0.0269(0.00157) & 0.000325(0.00247) & 1.24(0.0553) & 3.05(0.137) & 1.26(2.57) & 234(234) \\ 
  (1,1,1) & 500 & M & -0.0453(0.00149) & -0.00169(0.00193) & 1.12(0.0499) & 1.86(0.0833) & 1.13(2.63) & 206(206) \\ 
  (1,1,1) & 500 & Y & 0.111(0.00167) & 0.107(0.00192) & 1.4(0.0626) & 1.84(0.0823) & 1.44(2.08) & 268(268) \\ 
  (1,1,1) & 1000 & XYM & 0.00812(0.00112) & -0.00125(0.00122) & 1.25(0.0558) & 1.49(0.0669) & 1.26(3.39) & 644(644) \\ 
  (1,1,1) & 1000 & XY & 0.0115(0.00106) & -0.00175(0.00123) & 1.13(0.0505) & 1.51(0.0677) & 1.12(3.57) & 675(675) \\ 
  (1,1,1) & 1000 & XM & -0.0276(0.00111) & -0.000538(0.00162) & 1.23(0.0549) & 2.64(0.118) & 1.24(3.78) & 451(451) \\ 
  (1,1,1) & 1000 & M & -0.0464(0.00102) & -0.0035(0.00134) & 1.05(0.0469) & 1.81(0.0809) & 1.09(3.57) & 385(385) \\ 
  (1,1,1) & 1000 & Y & 0.113(0.0012) & 0.109(0.00141) & 1.45(0.0647) & 1.98(0.0888) & 1.44(2.92) & 529(529) \\ 
   \hline


==> plmed-paper arxiv/Plots/t/nde_tab.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Thu Jan  7 09:50:07 2021
Beta & N & Spec & Bias\_G & Bias\_TTS & Var\_G & Var\_TTS & Theory\_Var\_G & Boot\_Var\_G \\ 
  \hline
(0,0,0) & 100 & XYM & -0.00368(0.00703) & -0.00329(0.00757) & 4.95(0.221) & 5.73(0.256) & 4.8(0.0329) & 5.02(0.0354) \\ 
  (0,0,0) & 100 & XY & -0.0067(0.00723) & -0.00355(0.00782) & 5.22(0.234) & 6.11(0.273) & 4.8(0.0342) & 5(0.036) \\ 
  (0,0,0) & 100 & XM & 0.00277(0.00967) & 0.0136(0.0149) & 9.35(0.419) & 22.2(0.993) & 9.1(0.0968) & 9.44(0.097) \\ 
  (0,0,0) & 100 & M & 0.859(0.0106) & 0.946(0.0112) & 11.2(0.499) & 12.5(0.558) & 10.1(0.0966) & 10.5(0.0994) \\ 
  (0,0,0) & 100 & Y & 0.014(0.00713) & 0.0153(0.00731) & 5.09(0.228) & 5.34(0.239) & 4.7(0.029) & 4.87(0.0308) \\ 
  (0,0,0) & 500 & XYM & 0.000774(0.00305) & -0.000145(0.00323) & 4.65(0.208) & 5.23(0.234) & 4.81(0.0137) & 4.85(0.0154) \\ 
  (0,0,0) & 500 & XY & 0.00594(0.00324) & 0.00598(0.00343) & 5.24(0.234) & 5.87(0.263) & 4.83(0.0136) & 4.85(0.0155) \\ 
  (0,0,0) & 500 & XM & -0.00153(0.00435) & -0.00482(0.00808) & 9.45(0.423) & 32.7(1.46) & 9.63(0.0557) & 9.69(0.0565) \\ 
  (0,0,0) & 500 & M & 0.864(0.00459) & 0.947(0.00475) & 10.5(0.472) & 11.3(0.504) & 10.6(0.0526) & 10.7(0.0541) \\ 
  (0,0,0) & 500 & Y & -0.00428(0.00308) & -0.00494(0.00313) & 4.73(0.212) & 4.89(0.219) & 4.75(0.012) & 4.78(0.0138) \\ 
  (0,0,0) & 1000 & XYM & 0.000397(0.00226) & 0.00151(0.00238) & 5.12(0.229) & 5.65(0.253) & 4.83(0.00957) & 4.86(0.0116) \\ 
  (0,0,0) & 1000 & XY & -0.000543(0.00224) & -0.00172(0.00232) & 5(0.224) & 5.38(0.241) & 4.82(0.00953) & 4.83(0.012) \\ 
  (0,0,0) & 1000 & XM & 0.00162(0.00325) & 0.00184(0.00547) & 10.6(0.473) & 30(1.34) & 9.67(0.0395) & 9.7(0.0425) \\ 
  (0,0,0) & 1000 & M & 0.868(0.00323) & 0.948(0.00333) & 10.5(0.468) & 11.1(0.498) & 10.6(0.0381) & 10.7(0.0415) \\ 
  (0,0,0) & 1000 & Y & 0.00221(0.00214) & 0.00212(0.00218) & 4.58(0.205) & 4.73(0.212) & 4.76(0.0087) & 4.78(0.011) \\ 
  (1,1,1) & 100 & XYM & 0.012(0.00748) & 0.0165(0.0104) & 5.59(0.25) & 10.7(0.481) & 5.48(0.0399) & 5.76(0.0431) \\ 
  (1,1,1) & 100 & XY & 0.0157(0.00721) & 0.0209(0.00754) & 5.2(0.233) & 5.68(0.254) & 5.07(0.0358) & 5.29(0.0377) \\ 
  (1,1,1) & 100 & XM & 0.000393(0.0108) & -0.0156(0.0217) & 11.7(0.525) & 47.3(2.12) & 11(0.127) & 11.5(0.128) \\ 
  (1,1,1) & 100 & M & 0.849(0.0109) & 0.917(0.0166) & 11.9(0.532) & 27.6(1.24) & 11.7(0.133) & 12.2(0.136) \\ 
  (1,1,1) & 100 & Y & 0.00425(0.00763) & 0.0164(0.00931) & 5.82(0.261) & 8.66(0.388) & 5.47(0.0368) & 5.71(0.0393) \\ 
  (1,1,1) & 500 & XYM & 0.000856(0.00326) & -0.00715(0.0112) & 5.33(0.238) & 63.1(2.82) & 5.4(0.0175) & 5.45(0.0193) \\ 
  (1,1,1) & 500 & XY & -0.00366(0.00313) & -0.00349(0.00337) & 4.91(0.22) & 5.67(0.254) & 5.12(0.0148) & 5.16(0.0159) \\ 
  (1,1,1) & 500 & XM & 0.00671(0.0049) & -0.0199(0.0274) & 12(0.537) & 374(16.7) & 11.3(0.0617) & 11.3(0.0635) \\ 
  (1,1,1) & 500 & M & 0.862(0.00503) & 1.19(0.24) & 12.7(0.567) & 28800(1290) & 12.4(0.0697) & 12.5(0.0707) \\ 
  (1,1,1) & 500 & Y & -0.000415(0.00329) & -0.00134(0.00975) & 5.41(0.242) & 47.5(2.13) & 5.5(0.0164) & 5.53(0.018) \\ 
  (1,1,1) & 1000 & XYM & 0.00236(0.00228) & 0.0089(0.0455) & 5.21(0.233) & 2070(92.6) & 5.43(0.0119) & 5.46(0.0144) \\ 
  (1,1,1) & 1000 & XY & -0.000313(0.00221) & -0.00102(0.00234) & 4.87(0.218) & 5.48(0.245) & 5.1(0.0106) & 5.12(0.0129) \\ 
  (1,1,1) & 1000 & XM & 0.00758(0.00329) & 0.113(0.0773) & 10.8(0.483) & 5980(268) & 11.4(0.0459) & 11.5(0.048) \\ 
  (1,1,1) & 1000 & M & 0.864(0.00339) & 0.87(0.0548) & 11.5(0.513) & 3010(135) & 12.3(0.0469) & 12.3(0.0508) \\ 
  (1,1,1) & 1000 & Y & -0.000468(0.00235) & -0.199(0.221) & 5.51(0.247) & 49000(2190) & 5.5(0.0108) & 5.52(0.0133) \\ 
   \hline


==> plmed-paper arxiv/Plots/t/nide_tab.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Thu Jan  7 09:50:08 2021
Beta & N & Spec & Bias\_G & Bias\_TTS & Var\_G & Var\_TTS & Theory\_Var\_G & Boot\_Var\_G \\ 
  \hline
(0,0,0) & 100 & XYM & 0.000217(0.000709) & 0.00168(0.00121) & 0.0503(0.00225) & 0.147(0.00659) & 0.0984(0.00356) & 0.155(0.155) \\ 
  (0,0,0) & 100 & XY & 0.000536(0.000679) & 0.00193(0.00154) & 0.0461(0.00206) & 0.237(0.0106) & 0.0742(0.00289) & 0.117(0.117) \\ 
  (0,0,0) & 100 & XM & -0.000557(0.00124) & -0.00262(0.00261) & 0.154(0.00688) & 0.679(0.0304) & 0.285(0.0112) & 0.441(0.441) \\ 
  (0,0,0) & 100 & M & 0.000394(0.00114) & 0.0045(0.00231) & 0.13(0.00582) & 0.535(0.0239) & 0.242(0.0106) & 0.381(0.381) \\ 
  (0,0,0) & 100 & Y & -0.000822(0.0016) & -0.0018(0.00223) & 0.258(0.0115) & 0.498(0.0223) & 0.28(0.00735) & 0.332(0.332) \\ 
  (0,0,0) & 500 & XYM & 8.56e-05(0.000149) & 0.000237(0.000246) & 0.0111(0.000495) & 0.0302(0.00135) & 0.0196(0.000666) & 0.0296(0.0296) \\ 
  (0,0,0) & 500 & XY & 1.89e-05(0.000119) & 0.000217(0.000285) & 0.00702(0.000314) & 0.0407(0.00182) & 0.0141(0.000477) & 0.0213(0.0213) \\ 
  (0,0,0) & 500 & XM & 3.9e-05(0.000242) & -0.000221(0.000528) & 0.0293(0.00131) & 0.139(0.00624) & 0.0571(0.00189) & 0.0856(0.0856) \\ 
  (0,0,0) & 500 & M & 1.1e-05(0.000228) & 0.000383(0.000398) & 0.026(0.00116) & 0.0794(0.00355) & 0.0517(0.00181) & 0.0779(0.0779) \\ 
  (0,0,0) & 500 & Y & 0.000357(0.000675) & 0.000558(0.000943) & 0.228(0.0102) & 0.444(0.0199) & 0.222(0.00265) & 0.23(0.23) \\ 
  (0,0,0) & 1000 & XYM & 1.94e-05(7.09e-05) & -0.000156(0.000121) & 0.00502(0.000225) & 0.0146(0.000652) & 0.00985(0.000324) & 0.0148(0.0148) \\ 
  (0,0,0) & 1000 & XY & 4.19e-05(6.36e-05) & 7.49e-05(0.000152) & 0.00405(0.000181) & 0.023(0.00103) & 0.00729(0.000251) & 0.0108(0.0108) \\ 
  (0,0,0) & 1000 & XM & -0.000164(0.000122) & -4.87e-05(0.000261) & 0.0149(0.000665) & 0.0681(0.00305) & 0.0293(0.000969) & 0.044(0.044) \\ 
  (0,0,0) & 1000 & M & -0.000187(0.000119) & -0.000146(0.000199) & 0.0142(0.000636) & 0.0396(0.00177) & 0.0258(0.000902) & 0.0388(0.0388) \\ 
  (0,0,0) & 1000 & Y & -0.000691(0.000461) & -0.000609(0.000637) & 0.213(0.00953) & 0.406(0.0182) & 0.219(0.00194) & 0.223(0.223) \\ 
  (1,1,1) & 100 & XYM & -0.0104(0.00965) & -0.017(0.0121) & 9.3(0.416) & 14.6(0.652) & 8.7(0.11) & 9.09(9.09) \\ 
  (1,1,1) & 100 & XY & -0.0215(0.0116) & -0.0301(0.0175) & 13.4(0.6) & 30.5(1.36) & 12.6(0.145) & 12.9(12.9) \\ 
  (1,1,1) & 100 & XM & 0.00847(0.00995) & 0.00372(0.0188) & 9.89(0.443) & 35.2(1.57) & 9.97(0.128) & 10.6(10.6) \\ 
  (1,1,1) & 100 & M & -0.0017(0.00999) & 0.0244(0.0162) & 9.97(0.446) & 26.2(1.17) & 9.42(0.129) & 10(10) \\ 
  (1,1,1) & 100 & Y & 0.834(0.0119) & 0.906(0.0135) & 14.1(0.632) & 18.1(0.811) & 13.8(0.141) & 14.3(14.3) \\ 
  (1,1,1) & 500 & XYM & -0.0118(0.00416) & -0.00184(0.0116) & 8.65(0.387) & 67.8(3.04) & 8.61(0.0449) & 8.68(8.68) \\ 
  (1,1,1) & 500 & XY & 0.0018(0.00523) & -0.00395(0.00823) & 13.7(0.611) & 33.9(1.52) & 13.1(0.0755) & 13.2(13.2) \\ 
  (1,1,1) & 500 & XM & 0.000698(0.00445) & 0.0333(0.0266) & 9.89(0.443) & 353(15.8) & 9.88(0.0565) & 9.99(9.99) \\ 
  (1,1,1) & 500 & M & 0.00828(0.00433) & -0.238(0.24) & 9.37(0.419) & 28800(1290) & 9.39(0.0647) & 9.65(9.65) \\ 
  (1,1,1) & 500 & Y & 0.855(0.00529) & 0.938(0.0106) & 14(0.626) & 55.8(2.5) & 14.5(0.0749) & 14.6(14.6) \\ 
  (1,1,1) & 1000 & XYM & 0.00217(0.00298) & -0.00639(0.0457) & 8.9(0.398) & 2090(93.3) & 8.71(0.0361) & 8.75(8.75) \\ 
  (1,1,1) & 1000 & XY & -0.00308(0.00367) & -0.0062(0.00601) & 13.5(0.603) & 36.1(1.62) & 13.2(0.0548) & 13.2(13.2) \\ 
  (1,1,1) & 1000 & XM & 0.00129(0.00319) & -0.0985(0.0772) & 10.2(0.456) & 5960(267) & 9.84(0.0422) & 9.92(9.92) \\ 
  (1,1,1) & 1000 & M & -0.00305(0.00302) & 0.0711(0.055) & 9.12(0.408) & 3020(135) & 9.39(0.0538) & 9.55(9.55) \\ 
  (1,1,1) & 1000 & Y & 0.862(0.00374) & 1.14(0.221) & 14(0.624) & 49000(2190) & 14.7(0.0584) & 14.7(14.7) \\ 
   \hline

